Fisheye Camera and Ultrasonic Sensor Fusion For Near-Field Obstacle Perception in Bird's-Eye-View

Accurate obstacle identification represents a fundamental challenge within the scope of near-field perception for autonomous driving. Conventionally, fisheye cameras are frequently employed for comprehensive surround-view perception, including rear-view obstacle localization. However, the performance of such cameras can significantly deteriorate in low-light conditions, during nighttime, or when subjected to intense sun glare. Conversely, cost-effective sensors like ultrasonic sensors remain largely unaffected under these conditions. Therefore, we present, to our knowledge, the first end-to-end multimodal fusion model tailored for efficient obstacle perception in a bird's-eye-view (BEV) perspective, utilizing fisheye cameras and ultrasonic sensors. Initially, ResNeXt-50 is employed as a set of unimodal encoders to extract features specific to each modality. Subsequently, the feature space associated with the visible spectrum undergoes transformation into BEV. The fusion of these two modalities is facilitated via concatenation. At the same time, the ultrasonic spectrum-based unimodal feature maps pass through content-aware dilated convolution, applied to mitigate the sensor misalignment between two sensors in the fused feature space. Finally, the fused features are utilized by a two-stage semantic occupancy decoder to generate grid-wise predictions for precise obstacle perception. We conduct a systematic investigation to determine the optimal strategy for multimodal fusion of both sensors. We provide insights into our dataset creation procedures, annotation guidelines, and perform a thorough data analysis to ensure adequate coverage of all scenarios. When applied to our dataset, the experimental results underscore the robustness and effectiveness of our proposed multimodal fusion approach.

==> include/acknowledgement.tex <==
\section{Acknowledgement}

We would like to thank Valeo for encouraging advanced research. 

==> include/motivation.tex <==
\section{Motivation}




The endeavor to achieve reliable and accurate obstacle detection in the rear-view and close-proximity sensing \cite{eising2021near} domain carries considerable importance in the realm of autonomous vehicular navigation. This becomes of utmost importance due to the vital factors associated with efficiency and safety of autonomous vehicles. The capability to accurately identify and distinguish obstacles, particularly those positioned at lower elevations or ground-level locations is one of the most important aspect to ensure safety of autonomous vehicles. This capability safeguards the welfare of vulnerable road users, including pedestrians and cyclists, while also ensuring the safety of other vehicles sharing the roadway. In urban settings marked by the close interplay between vehicles and pedestrians, the precise detection and tracking of obstacles emerge as indispensable measures to mitigate the risk of potential accidents and collisions. Additionally, for maintaining a stable vehicle movement trajectory and maneuverability, the recognition of low-lying obstacles such as debris, vegetation, cartons, or bottles is of great significance. Moreover, the implementation of a robust rear-view obstacle perception system enhances the holistic situational awareness of autonomous vehicles, enabling them to make well-informed decisions and execute prudent maneuvers when encountering obstacles within their trajectory. This comprehensive strategy, serves as a cornerstone for the achievement of safer, more reliable, and highly efficient autonomous driving experiences. Figure \ref{fig:different_obstacles} shows several instances of commonly encountered obstacles in rear-view.



